Optimization-Based Quadrupedal Hybrid Wheeled-Legged Locomotion

Hybrid wheeled-legged locomotion is a navigation paradigm only recently opened up by novel robotic designs,e.g. the centaur-type humanoid CENTAURO [1] or the quadruped ANYmal [2] in its configuration featuring non-steerable wheels. The term Hybrid Locomotion is hereafter used to indicate a particular type of locomotion, achieved with simultaneous and coordinate use of legs and wheels,see Fig. 1. Such choice stems at the intersection between legged locomotion and the simpler wheeled navigation, in order to get the best from both techniques: agility and ability to traverse uneven terrains from the first, speed and stability from the second. As a consequence, the problem of planning feasible trajectories for a hybrid robot shares many similarities with the legged locomotion problem: also in the hybrid case the motion of the base is reached through contact of the feet with the environment, taking into account that the wheeled feet can just push on the ground and not pull it. Forces compatible with friction cones have to be considered, while the contacts can slide just along the direction prescribed by the orientation of the wheels.

==> intro_legged.tex <==
\subsubsection{Legged locomotion}
Two main approaches can be taken while planning trajectories for such robots, namely Dynamic Programming (DP) or Trajectory Optimization (TO). Both approaches are concerned in casting a continuous time Optimal Control (OC) problem into a more manageable discrete time one. DP-based solutions arise from the Bellman optimality principle and have the need to represent all the possible states in which the system can exist together with how the system evolves from those, given the different inputs. In a highly complex and nonlinear framework such as legged robotics, it has been believed for long that DP does not scale well because of the curse of dimensionality. Recently, newly developed processors and improvement in algorithmic theory have awakened the efforts in this field, where interesting results are brought in quadrupedal locomotion and planning by the works in \cite{farshidian2017efficient, 7845678}. TO-based approaches use Direct Methods to cast the OC problem into a finite dimensional Non-Linear Programming (NLP) problem, and once this conversion is done only the latter needs to be solved, usually resorting to off-the-shelf structure exploiting numerical algorithms like Ipopt \cite{ipopt}. As the search space that these methods need to explore is quite large, they have often been implemented into separate sub-problems where base and feet motion are solved separately. Even if such a choice leads to interesting results in \cite{LQR_method} and \cite{kalakrishnan2011learning}, where respectively pre-planned foot positions or footholds learnt by expert demonstrations are adopted, it decouples two inherently related quantities. A more general approach consists of fixing in advance just the timings in which each foot must be in contact with the ground, while leaving to the optimizer the task to decide the optimal position for them. This approach proves to be fast computationally and has been successfully tested on a real robot in \cite{wink1stpaper}, and for these reasons is the one that most resembles the presented approach in the first part of our paper. Very recent results expanded the flexibility of TO by defining just the sequence in which the feet should be moved or even letting the optimizer free to choose the best gait sequence to adopt, leading to results in which flight phases are reached as demonstrated in \cite{wink3rdpaper}.

\subsubsection{Hybrid locomotion}

\subsection{Contribution}



\dots \cite{muratore2017xbotcore, OpenSot17}
